Content-aware Neural Hashing for Cold-start Recommendation

Content-aware recommendation approaches are essential for providing meaningful recommendations for \textit{new} (i.e., \textit{cold-start}) items in a recommender system. We present a content-aware neural hashing-based collaborative filtering approach (NeuHash-CF), which generates binary hash codes for users and items, such that the highly efficient Hamming distance can be used for estimating user-item relevance. NeuHash-CF is modelled as an autoencoder architecture, consisting of two joint hashing components for generating user and item hash codes. Inspired from semantic hashing, the item hashing component generates a hash code directly from an item's content information (i.e., it generates cold-start and seen item hash codes in the same manner). This contrasts existing state-of-the-art models, which treat the two item cases separately. The user hash codes are generated directly based on user id, through learning a user embedding matrix. We show experimentally that NeuHash-CF significantly outperforms state-of-the-art baselines by up to 12\% NDCG and 13\% MRR in cold-start recommendation settings, and up to 4\% in both NDCG and MRR in standard settings where all items are present while training. Our approach uses 2-4x shorter hash codes, while obtaining the same or better performance compared to the state of the art, thus consequently also enabling a notable storage reduction.

==> Content-aware Neural Hashing for Collaborative Filtering (1)/tables/coldres.tex <==
\begin{table*}[]
    \centering
        \caption{NDCG@10 and MRR scores for 32 dimensional representations in varying cold-start scenarios with 10-50\% of the items used for training. Bold numbers represent the best hashing-based approach and statistically significant results compared to the best hashing-based baseline in each column are marked with a star.}
        \vspace{-9pt}
    \scalebox{0.76}{
    \begin{tabular}{@{}lll|ll|ll|ll|ll|ll|ll|ll|ll|ll@{}}
    \toprule
      &  \multicolumn{10}{c|}{Yelp (out-of-matrix)} & \multicolumn{10}{c}{Amazon (out-of-matrix)} \\ 
      & \multicolumn{2}{c}{10\%} & \multicolumn{2}{c}{20\%} & \multicolumn{2}{c}{30\%} & \multicolumn{2}{c}{40\%} & \multicolumn{2}{c|}{50\%} & \multicolumn{2}{c}{10\%} & \multicolumn{2}{c}{20\%} & \multicolumn{2}{c}{30\%} & \multicolumn{2}{c}{40\%} & \multicolumn{2}{c}{50\%} \\
    NDCG & \small @10 & \small MRR & \small @10 & \small MRR & \small @10 & \small MRR & \small @10 & \small MRR & \small @10 & \small MRR & \small @10 & \small MRR & \small @10 & \small MRR & \small @10 & \small MRR & \small @10 & \small MRR & \small @10 & \small MRR \\
    \toprule
NeuHash-CF & \textbf{.730}$^*$ & \textbf{.603}$^*$ & \textbf{.750}$^*$ & \textbf{.634}$^*$ & \textbf{.769}$^*$ & \textbf{.666}$^*$ & \textbf{.771}$^*$ & \textbf{.668}$^*$ & \textbf{.772}$^*$ & \textbf{.674}$^*$ & \textbf{.794}$^*$ & \textbf{.727}$^*$ & \textbf{.812}$^*$ & \textbf{.753}$^*$ & \textbf{.817}$^*$ & \textbf{.761}$^*$ & \textbf{.818}$^*$ & \textbf{.763}$^*$ & \textbf{.818}$^*$ & \textbf{.764}$^*$ \\
DCMF & .688 & .572 & .693 & .578 & .704 & .593 & .710 & .602 & .709 & .604 & .774 & .710 & .778 & .712 & .781 & .717 & .784 & .720 & .784 & .721 \\
DDL & .678 & .556 & .681 & .562 & .687 & .572 & .684 & .571 & .681 & .562 & .770 & .713 & .766 & .689 & .767 & .700 & .765 & .693 & .767 & .694 \\
\midrule
FM (real-valued) & .766$^*$ & .688$^*$ & .776$^*$ & .707$^*$ & .778$^*$ & .712$^*$ & .786$^*$ & .724$^*$ & .785$^*$ & .722$^*$ & .806$^*$ & .759$^*$ & .813$^*$ & .771$^*$ & .817$^*$ & .775$^*$ & .823$^*$ & .786$^*$ & .821$^*$ & .784$^*$ \\
\bottomrule
    \end{tabular}}

    \label{tab:cold_res}
    \vspace{-7pt}
\end{table*}


==> Content-aware Neural Hashing for Collaborative Filtering (1)/tables/mainmrr.tex <==
\begin{table*}[]
    \centering
        \caption{MRR scores in both in-matrix and out-of-matrix settings. Bold numbers represent the best hashing-based approach and statistically significant results compared to the best hashing-based baseline per column are marked with a star. Dashed lines correspond to not content-aware approaches in out-of-matrix setting.}
        \vspace{-6pt}
    \scalebox{0.99}{
    \begin{tabular}{@{}llll|lll|lll|lll@{}}
    \toprule
      & \multicolumn{3}{c|}{Yelp (in-matrix)} & \multicolumn{3}{c|}{Yelp (out-of-matrix)} & \multicolumn{3}{c|}{Amazon (in-matrix)} & \multicolumn{3}{c}{Amazon (out-of-matrix)}\\ 
    MRR & \small 16 dim. & \small 32 dim. & \small 64 dim. & \small 16 dim. & \small 32 dim. & \small 64 dim. & \small 16 dim. & \small 32 dim. & \small 64 dim. & \small 16 dim. & \small 32 dim. & \small 64 dim. \\
      \toprule
NeuHash-CF & \textbf{.646}$^*$ & \textbf{.668}$^*$ & \textbf{.687}$^*$ & \textbf{.628}$^*$ & \textbf{.674}$^*$ & \textbf{.692}$^*$ & \textbf{.749}$^*$ & \textbf{.770}$^*$ & \textbf{.779}$^*$ & \textbf{.750}$^*$ & \textbf{.764}$^*$ & \textbf{.782}$^*$ \\
DCMF & .629 & .644 & .660 & .598 & .604 & .612 & .738 & .753 & .767 & .719 & .721 & .726 \\
DDL & .620 & .638 & .651 & .557 & .562 & .604 & .721 & .741 & .753 & .696 & .694 & .694 \\
\midrule
NeuHash-CF/no.C & .621 & .642 & .656 & - & - & - & .737 & .752 & .764 & - & - & - \\
DCF & .626 & .636 & .664 & - & - & - & .736 & .751 & .769 & - & - & - \\
\midrule
MF (real-valued) & .767$^*$ & .767$^*$ & .767$^*$ & - & - & - & .826$^*$ & .826$^*$ & .826$^*$ & - & - & - \\
FM (real-valued) & .761$^*$ & .756$^*$ & .750$^*$ & .730$^*$ & .722$^*$ & .717$^*$ & .824$^*$ & .821$^*$ & .815$^*$ & .792$^*$ & .784$^*$ & .780$^*$ \\ \bottomrule
    \end{tabular}}
    \label{tab:mainres_mrr}
    \vspace{-6pt}
\end{table*}

==> Content-aware Neural Hashing for Collaborative Filtering (1)/tables/mainres.tex <==

\begin{table*}[]
    \centering
    \caption{NDCG@k scores on in-matrix and out-of-matrix settings for the Amazon and Yelp datasets. Bold numbers represent the best hashing-based approach and statistically significant results compared to the best hashing-based baseline per column are marked with a star. Dashed lines correspond to not content-aware approaches in out-of-matrix setting.}
    \vspace{-6pt}
    \scalebox{0.825}{
    \begin{tabular}{@{}llll|lll|lll|lll|lll|lll@{}}
    \toprule
      & \multicolumn{9}{c|}{Yelp (in-matrix)} & \multicolumn{9}{c}{Yelp (out-of-matrix)}\\ 
      & \multicolumn{3}{c|}{16 dim.} & \multicolumn{3}{c|}{32 dim.} & \multicolumn{3}{c|}{64 dim.} &  \multicolumn{3}{c|}{16 dim.} & \multicolumn{3}{c|}{32 dim.} & \multicolumn{3}{c}{64 dim.} \\ 
      NDCG & @2 & @6 & @10 & @2 & @6 & @10 & @2 & @6 & @10 & @2 & @6 & @10 & @2 & @6 & @10 & @2 & @6 & @10 \\
      \toprule
NeuHash-CF & \textbf{.662}$^*$ & \textbf{.701}$^*$ & \textbf{.752}$^*$ & \textbf{.681}$^*$ & \textbf{.718}$^*$ & \textbf{.766}$^*$ & \textbf{.697}$^*$ & \textbf{.731}$^*$ & \textbf{.776}$^*$ &  \textbf{.646}$^*$ & \textbf{.694}$^*$ & \textbf{.747}$^*$ & \textbf{.687}$^*$ & \textbf{.725}$^*$ & \textbf{.772}$^*$ & \textbf{.702}$^*$ & \textbf{.737}$^*$ & \textbf{.780}$^*$ \\
DCMF & .642 & .678 & .733 & .655 & .691 & .743 & .670 & .701 & .752 &  .611 & .647 & .703 & .617 & .655 & .709 & .626 & .664 & .717 \\
DDL & .636 & .674 & .729 & .651 & .686 & .739 & .664 & .698 & .749 &  .575 & .615 & .673 & .579 & .622 & .681 & .612 & .646 & .700 \\
\midrule
NeuHash-CF/no.C & .634 & .672 & .727 & .655 & .689 & .741 & .666 & .699 & .749 &  - & - & - & - & - & - & - & - & - \\
DCF & .639 & .676 & .730 & .649 & .685 & .738 & .671 & .700 & .750 &  - & - & - & - & - & - & - & - & - \\
\midrule
MF (real-valued) & .755$^*$ & .763$^*$ & .800$^*$ & .755$^*$ & .763$^*$ & .800$^*$ & .755$^*$ & .763$^*$ & .800$^*$ &  - & - & - & - & - & - & - & - & - \\
FM (real-valued) & .754$^*$ & .763$^*$ & .801$^*$ & .750$^*$ & .760$^*$ & .798$^*$ & .744$^*$ & .755$^*$ & .794$^*$ &  .731$^*$ & .750$^*$ & .789$^*$ & .724$^*$ & .744$^*$ & .785$^*$ & .719$^*$ & .740$^*$ & .781$^*$ \\
\bottomrule
%\vspace{5pt}
    \end{tabular}}
    \centering
    \scalebox{0.825}{
    \begin{tabular}{@{}llll|lll|lll|lll|lll|lll@{}}
   % \toprule
      & \multicolumn{9}{c|}{Amazon (in-matrix)} & \multicolumn{9}{c}{Amazon (out-of-matrix)}\\ 
      & \multicolumn{3}{c|}{16 dim.} & \multicolumn{3}{c|}{32 dim.} & \multicolumn{3}{c|}{64 dim.} &  \multicolumn{3}{c|}{16 dim.} & \multicolumn{3}{c|}{32 dim.} & \multicolumn{3}{c}{64 dim.} \\ 
    NDCG & @2 & @6 & @10 & @2 & @6 & @10 & @2 & @6 & @10 & @2 & @6 & @10 & @2 & @6 & @10 & @2 & @6 & @10 \\
      \toprule
NeuHash-CF & \textbf{.759}$^*$ & \textbf{.777}$^*$ & \textbf{.810}$^*$ & \textbf{.780}$^*$ & \textbf{.798}$^*$ & \textbf{.827}$^*$ & \textbf{.786}$^*$ & \textbf{.803}$^*$ & \textbf{.831}$^*$ &  \textbf{.758}$^*$ & \textbf{.778}$^*$ & \textbf{.809}$^*$ & \textbf{.769}$^*$ & \textbf{.788}$^*$ & \textbf{.818}$^*$ & \textbf{.787}$^*$ & \textbf{.804}$^*$ & \textbf{.831}$^*$ \\
DCMF & .749 & .767 & .800 & .761 & .777 & .810 & .773 & .788 & .818 &  .727 & .748 & .782 & .729 & .749 & .784 & .733 & .752 & .786 \\
DDL & .734 & .755 & .791 & .748 & .768 & .802 & .762 & .779 & .811 &  .704 & .728 & .766 & .705 & .729 & .767 & .705 & .727 & .766 \\
\midrule
NeuHash-CF/no.C & .748 & .768 & .802 & .760 & .776 & .808 & .771 & .785 & .816 &  - & - & - & - & - & - & - & - & - \\
DCF & .745 & .767 & .802 & .759 & .776 & .809 & .774 & .787 & .818 &  - & - & - & - & - & - & - & - & - \\
\midrule
MF (real-valued) & .824$^*$ & .826$^*$ & .848$^*$ & .824$^*$ & .826$^*$ & .848$^*$ & .824$^*$ & .826$^*$ & .848$^*$ &  - & - & - & - & - & - & - & - & - \\
FM (real-valued) & .821$^*$ & .822$^*$ & .845$^*$ & .817$^*$ & .819$^*$ & .843$^*$ & .813$^*$ & .816$^*$ & .841$^*$ &  .792$^*$ & .800$^*$ & .827$^*$ & .785$^*$ & .793$^*$ & .821$^*$ & .780$^*$ & .790$^*$ & .819$^*$ \\
\bottomrule
    \end{tabular}}
    \label{tab:mainres_ndcg}
    \vspace{-6pt}
\end{table*}

